Neural Variational Inference For Estimating Uncertainty in Knowledge Graph Embeddings

Recent advances in Neural Variational Inference allowed for a renaissance in latent variable models in a variety of domains involving high-dimensional data. While traditional variational methods derive an analytical approximation for the intractable distribution over the latent variables, here we construct an inference network conditioned on the symbolic representation of entities and relation types in the Knowledge Graph, to provide the variational distributions. The new framework results in a highly-scalable method. Under a Bernoulli sampling framework, we provide an alternative justification for commonly used techniques in large-scale stochastic variational inference, which drastically reduce training time at a cost of an additional approximation to the variational lower bound. We introduce two models from this highly scalable probabilistic framework, namely the Latent Information and Latent Fact models, for reasoning over knowledge graph-based representations. Our Latent Information and Latent Fact models improve upon baseline performance under certain conditions. We use the learnt embedding variance to estimate predictive uncertainty during link prediction, and discuss the quality of these learnt uncertainty estimates. Our source code and datasets are publicly available online at https://github.com/alexanderimanicowenrivers/Neural-Variational-Knowledge-Graphs.

==> DASA.tex <==
%!TEX root = ../ijcai19.tex

\subsection{Opponent Modeling}
\label{sec:AOM}
In this section, we focus on modeling the opponents actions, a.k.a the market price distribution. The opponent model is defined as the market price distribution at an impression level. We use $a_{-i}$ to represent the action taken by the opponents, a.k.a the highest price from all the other participants in the auction. In this study, $a_{-i}=z$, where $z$ is the market price. The probability density function (P.D.F) of $z$ is $p_{z}(z)$.

\begin{equation}\label{eq:pr}
    p_{z}(z) = P(a_{-i}=z | x, \theta) = h_{z} \prod_{j<z}(1-h_{j})
\end{equation}

As is shown in Eq. \ref{eq:pr}, the P.D.F of the market price can be calculated from the instant hazard function $h_{j}$ which indicates the probability of the instant occurrence of the event at time $j$ conditioned on the event has not happened prior to time $j$. In the RTB setting, $\prod_{j<z}(1-h_{j})$ represents the losing probability of bidding less than the market price and $h_{z}$ shows the probability of observing the market price $z$.

We take the features in the bid request as input and predict the hazard function $h$ over the discretized bid price space at each impression level. The $p_{z}$ can be easily derived from Eq.~\ref{eq:pr}. For the uncensored data, the true label is an one-hot encoded vector of size $b_{max}$ with the element indexed by the market price as 1. 
%We followed the loss functions in \cite{ren2019deep} and trained the transformer model.
%as is shown in~\ref{fig:DASA}.

% For this work, we only employ only the encoding component of the Transformer architecture. The encoder is a stack of six identical layers. Each layer has two sub-layers. The first is a multi-head attention mechanism, the second is a simple fully connected feed-forward network. Residual connections~\cite{he2016deep} are used around each of the two sub-layers, followed by layer normalization~\cite{ba2016layer}. The output of each sub-layer can be given by the equation

% \begin{equation*}
% \begin{array}{cc}
%      & F(x) = LayerNorm(x + Sublayer(x))
% \end{array}
% \end{equation*}

% All sub-layers in the model  produce outputs of dimension $512$ in order to facilitate residual connections. 

% The type of attention used is referred to as a scaled-dot product attention, whereby the scaling factor $\frac{1}{\sqrt{d}_k}$ is used to combat the dot products pushing the softmax function into regions of small gradient.  

% \begin{equation*}
% \begin{array}{cc}
%      & Attention(Q, K, V ) = \text{softmax}(\frac{QKT}{\sqrt{d}_k})V
% \end{array}
% \end{equation*}

% The transformer employs multi-head attention, which uses a projection trick to attend to multiple parts of an input with the same computation cost as one full dimensional attention. 

% \begin{equation*}
% \begin{array}{cc}
%      & MultiHead(Q, K, V ) = Concat(head1, ..., headh)W_O \\
%      & \text{where } headi = Attention(QW^Q_i,KW^K_i,VW^V_i) \\
%      & \text{and } W_O \in \mathbb{R}^{512,512}
% \end{array}
% \end{equation*}

% Where $W^Q_i,W^K_i,W^V_i \in \mathbb{R}^{512,d_k}$ are projection matrices which project onto $d_k=64$ dimensions.
%
%\begin{figure}[t!]
%\includegraphics[scale=0.25]{figures/Architecture.pdf}
%\caption{The architecture of the Deep Attentive Survival model. Where N is the number of stacks.}\label{fig:DASA}
%\end{figure}

% We also employ the positional encoding, with the size equal to the dimension of the Transformer \cite{vaswani2017attention}.

% $$
% \begin{aligned}
%     \text{PE}_{(pos, 2i)} = \sin (pos/10000^{2i/d_{\text{model}}}) \\ 
%     \text{PE}_{(pos, 2i+1)} = \cos (pos/10000^{2i/d_{\text{model}}})
% \end{aligned}
% $$

%After the feeding in the features to the model, it will output the Tensor with shape: [batch size x sequence length x model dimension]. Finally, the training loss is calculated according to ~\cite{ren2019deep}.


We followed the loss functions in \cite{ren2019deep}, for the uncensored data, the loss of the observed market price is defined as:
\begin{align}\label{eq:Lz}
L_{z} = -\sum_{x, a_{-i} \in \mathcal{D}_{\text{uncensored}}}[log h_{z} + \sum_{j<z}log(1-h_{j})] \nonumber
\end{align}

For the censored data, it is certain to still lose the auction by bidding lower than the current price. The corresponding loss is defined as:
$$
\begin{aligned}
L_{\text{censored}}
      = -\sum_{x, a_{i} \in \mathcal{D}_{\text{censored}}}\sum_{j<a_{i}} log(1-h_{j}) \nonumber
\end{aligned}
$$

In addition, for the winning auctions, by bidding at any price higher than the observed market price, it is guaranteed to win the auction.
Such information can be shared with the censored data. The loss function is defined as followed:
$$
\begin{aligned}
L_{\text{uncensored}} 
      = -\sum_{x, a_{i} \in \mathcal{D}_{\text{uncensored}}}log[1 - \prod_{j<a_{i}}(1-h_{j})] \nonumber
\end{aligned}
$$

The total loss of the model takes the combination of the above losses as below where $\alpha$ balances the loss values. 
$$
\begin{aligned}
L_{\text{total}}= \alpha L_{z} + (1 - \alpha)(L_{\text{censored}} + L_{\text{uncensored}})
\end{aligned}
$$

%The loss composed of 3 parts (equation taken fron \cite{ren2019deep})
%
%\begin{itemize}
%  \item Maximize the log-likelihood of true event time.
%    $$
%    \begin{aligned}
%    L_z = - \sum_{(\bold{x}^i, z^i) \in \mathbb{D}_{\text{uncensored}}} \left[ \log h^i_{l^i}  + \sum_{l: l < l^i} \log(1 - h^i_l)  \right] ~,
%    \end{aligned}
%    $$
%    
%  \item Maximize the partial log-likelihood of event rate in unsensored data.
%    $$
%    \begin{aligned}
%    L_{\text{uncensored}}= - \sum_{(\bold{x}^i, t^i) \in \mathbb{D}_{\text{uncensored}}} \log \Big[ 1- \prod_{l: l \leq l^i} (1 - h^i_l) \Big] ~.
%    \end{aligned}
%    $$
%  \item Partial log-liklihood on censored data, since we at least know that the event happend after our logged time. 
%    $$
%    \begin{aligned}
%    L_{\text{censored}} = - \sum_{(\bold{x}^i, t^i) \in \mathbb{D_{\text{censored}}}} \sum_{l: l \leq l^i} \log (1 - h^i_l) ~.
%    \end{aligned}
%    $$
%\end{itemize}
%
%Where $h_i$ is the output probabilities from the model after passing through sigmoid function $\sigma$. Finally, DASA optimizes the objective: 
%$$
%\begin{aligned}
%    \arg\min_{\theta} \alpha L_z &+ (1-\alpha) L_{\text{c}} \\
%    &\text{ where } L_{\text{c}} = L_{\text{uncensored}} + L_{\text{censored}}
%\end{aligned}
%$$


